Attributes2Classname: A discriminative model for attribute-based unsupervised zero-shot learning

We propose a novel approach for unsupervised zero-shot learning (ZSL) of classes based on their names. Most existing unsupervised ZSL methods aim to learn a model for directly comparing image features and class names. However, this proves to be a difficult task due to dominance of non-visual semantics in underlying vector-space embeddings of class names. To address this issue, we discriminatively learn a word representation such that the similarities between class and combination of attribute names fall in line with the visual similarity. Contrary to the traditional zero-shot learning approaches that are built upon attribute presence, our approach bypasses the laborious attribute-class relation annotations for unseen classes. In addition, our proposed approach renders text-only training possible, hence, the training can be augmented without the need to collect additional image data. The experimental results show that our method yields state-of-the-art results for unsupervised ZSL in three benchmark datasets.

==> Makefile <==
######################################################################
# Makefile for compiling tex files and setting up sharing permissions.
# Last edit: Gokberk Cinbis, 2013-10-07.

# Constants to be read from Makefile.mk
# TEXFILE=<tex filename>
# TITLE=<project title>

# Environment variables (unless overriden by input file)
# PDFDIR: Optional environment variable for output files.

######################################################################

include Makefile.mk

#PDFDIR= ## !!!!

# if PDFDIR is undefined OR '', then use the current directory.
PDFDIR?=.
ifeq "$(PDFDIR)" ""
    PDFDIR=.
endif
ifneq "$(PDFDIR)" "."
    PDFDIR:=$(PDFDIR)/$(TITLE)
endif

CMDPDFMAIN=pdflatex -output-directory $(PDFDIR) $(TEXFILE)
CMDPDF=$(CMDPDFMAIN) -file-line-error -interaction=nonstopmode | grep -i -e warn -e error -e pages -B4 -A4 -e '^l.' -e '^?' # hangs in cygwin in interactive mode
#CMDPDF=$(CMDPDFMAIN) -interaction=nonstopmode

#all:	export pdf bib share echo 
all:	pdfnonstop bib echo 
	cp -f $(PDFDIR)/$(TEXFILE:.tex=.pdf) .

warn:	pdfnonstopwarnonly 

error:	pdferror bib echo

sup:	
	pdflatex supmat.tex
	bibtex supmat

echo:
	echo "Tex file: $(TEXFILE)"
	echo "Output files are under: $(PDFDIR)"

view:	all
	$(PDFVIEW) $(PDFDIR)/$(TEXFILE:.tex=.pdf) &

open:	
	$(OPEN) $(PDFDIR) &

ps:	$(TEXFILE:.tex=.ps)
dvi:	$(TEXFILE:.tex=.dvi)
bib:	pdfnonstop bibrule

alf:
	echo "-$(PDFDIR)-"

bibrule:	$(TEXFILE)
	( \
	echo ================= bib ======================; \
	export openout_any=a; \
	bibtex "$(PDFDIR)/$(<:.tex=)"; \
	)

%.dvi: %.tex checkdep
	( \
	echo ================= latex ======================; \
	latex $<; \
	while grep -q "Rerun to get cross-references right." $(<:.tex=.log); \
	do \
		echo ================= latex loop ======================; \
		latex $<; \
	done \
	)

%.ps: %.dvi
	dvips -q -t a4 $< -o $(<:.dvi=.ps)

latex:	$(TEXFILE:.tex=.ps)
	ps2pdf -dPDFSETTINGS=/prepress $<

# Note: $< is the first dependency.
#
# pdflatex -interaction=batchmode -halt-on-error -file-line-error $(TEXFILE); 
# use "X" to quit.
# 
# output-directory should be before the filename.
# pdflatex -file-line-error -output-directory $(PDFDIR) $(<); 
#
# Don't stop on errors
pdfnonstop:$(TEXFILE) checkdep 
	( \
	echo ================= pdflatex ======================; \
	mkdir -p $(PDFDIR); \
	$(CMDPDF); \
	while grep -q "Rerun to get" $(PDFDIR)/$(<:.tex=.log); \
	do \
		echo ================= pdflatex loop ======================; \
		$(CMDPDF); \
	done \
	)

# Don't stop on errors, show warnings only
pdfnonstopwarnonly:$(TEXFILE) checkdep 
	( \
	echo ================= pdflatex ======================; \
	mkdir -p $(PDFDIR); \
	$(CMDPDF) | grep Warn; \
	while grep -q "Rerun to get" $(PDFDIR)/$(<:.tex=.log); \
	do \
		echo ================= pdflatex loop ======================; \
		$(CMDPDF) | grep Warn; \
	done \
	)


# Stop on errors
pdferror: 	$(TEXFILE) checkdep 
	( \
	echo ================= pdflatex ======================; \
	mkdir -p $(PDFDIR); \
	$(CMDPDFMAIN); \
	while grep -q "Rerun to get" $(PDFDIR)/$(<:.tex=.log); \
	do \
		echo ================= pdflatex loop ======================; \
		$(CMDPDFMAIN); \
	done \
	)

compress:
	(cd $(PDFDIR) && ls -alh $(TEXFILE:.tex=.pdf) && pdf2ps $(TEXFILE:.tex=.pdf) && ps2pdf $(TEXFILE:.tex=.ps) && ls -alh $(TEXFILE:.tex=.pdf) && rm -f ps2pdf $(TEXFILE:.tex=.ps))

share:	
	find . -user ${USER} -type d -execdir chmod 770 "{}" \;
	find . -user ${USER} -type f -execdir chmod 660 "{}" \;

# check whether bibtex changed the bibliography file
checkdep: $(TEXFILE:.tex:.aux) 

export:	
	bash export.sh

clean:
	@rm -f {./,$(PDFDIR)/}$(TEXFILE:.tex=.){aux,log,out,dvi,pdf,bbl,blg,ps,brf,lof,lot,nlo,maf,toc} 
	@rm -f {./,$(PDFDIR)/}$(TEXFILE:.tex=.){mlc,mlt,mtc,mlf}*



==> macros.tex <==
% based on Jakob Verbeek's macros.tex

\usepackage{color}
\usepackage[normalem]{ulem}

\def\etal{et al.\ }
\def\Eq#1{Eq.~(\ref{eq:#1})}

\usepackage{amsmath,amssymb,amsbsy,xspace}
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{c.f}\onedot} \def\Cf{\emph{C.f}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot} 
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\etal{\emph{et al}\onedot}

\def\Eqs#1{Eqs.~(\ref{eq:#1})}
\def\Eq#1{Eq.~(\ref{eq:#1})}
\def\eq#1{(\ref{eq:#1})}
\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\bea{\begin{eqnarray}}
\def\eea{\end{eqnarray}}
\def\fig#1{Figure~\ref{fig:#1}}
\def\tab#1{Table~\ref{tab:#1}}
\def\sect#1{Section~\ref{sec:#1}}
\def\chap#1{Chapter~\ref{chap:#1}}
\def\app#1{Appendix~\ref{app:#1}}
\def\algo#1{Algorithm~\ref{algo:#1}}

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
%\newcommand{\argmin}{\operatornamewithlimits{argmin}}
%\newcommand{\argmax}{\operatornamewithlimits{argmax}}

\makeatother



==> table_big.tex <==
\begin{table*}[th]
\begin{center}
\caption{Zero-shot learning results of various unsupervised and supervised methods on two different datasets. The approaches mentioned below include different deep visual features such as CNN-M2K\textsuperscript{a}, GoogleNet\textsuperscript{b} and VGG-19\textsuperscript{c}.}
\label{table:comparisonSOA}
\begin{tabularx}{480pt}{lcccccll}
\hline
Method & \multicolumn{3}{c}{Training Phase} & \multicolumn{2}{c}{Testing Phase} & \multicolumn{2}{l}{Accuracy}                         \\
\hline
                                                                   & \multicolumn{1}{l}{Visual Features} & \multicolumn{1}{l}{Attributes} & \multicolumn{1}{l}{Textual Corpus} & \multicolumn{1}{l}{Attributes} & \multicolumn{1}{l}{Textual Corpus} & AwA                               & aPaY      \\
       \hline
 & \multicolumn{7}{c}{Unsupervised Methods}                                                                                                                                                    \\
       \hline
ALE\cite{akata2015evaluation}\textsuperscript{a}                   & $\surd$                             &                                & $\surd$                            &                                & $\surd$                            & \multicolumn{1}{c}{59.8}          & \multicolumn{1}{c}{33.3}  \\
LatEM\cite{xian2016latent}\textsuperscript{b}                      & $\surd$                             &                                & $\surd$                            &                                & $\surd$                            & \multicolumn{1}{c}{62.9}          & \multicolumn{1}{c}{-}     \\
DeViSE\cite{frome2013devise}\textsuperscript{b}                    & $\surd$                             &                                &                                    &                                & $\surd$                            & \multicolumn{1}{c}{44.5}          & \multicolumn{1}{c}{25.5}  \\
ConSE\cite{norouzi2013zero}\textsuperscript{b}                     & $\surd$                             &                                &                                    &                                & $\surd$                            & \multicolumn{1}{c}{46.1}          & \multicolumn{1}{c}{22.0}  \\
Text2Visual\cite{elhoseiny2013write,bo2010twin}\textsuperscript{b} & $\surd$                             &                                & $\surd$                            &                                & $\surd$                            & 55.3                              & 30.2                      \\
CAAP\cite{al2016recovering}\textsuperscript{b}                     &                                     & $\surd$                        & $\surd$                            &                                & $\surd$                            & \multicolumn{1}{c}{67.5}          & \multicolumn{1}{c}{37.0}  \\

PBW - word2vec\textsuperscript{a}                                  &                                     & $\surd$                        & $\surd$                            &                                & $\surd$                            & 69.1                              & 37.1                    \\
IBW - word2vec\textsuperscript{a}                                  & $\surd$                             & $\surd$                        & $\surd$                            &                                & $\surd$                            & 67.1                              & 35.0                     \\
PBW - GloVe\textsuperscript{a}                                     &                                     & $\surd$                        & $\surd$                            &                                & $\surd$                            & 60.7                              & 29.4                     \\
IBW - GloVe\textsuperscript{a}                                     & $\surd$                             & $\surd$                        & $\surd$                            &                                & $\surd$                            & \textbf{69.8}                     & \textbf{38.2}            \\
                                                                   & \multicolumn{1}{l}{}                & \multicolumn{1}{l}{}           & \multicolumn{1}{l}{}               & \multicolumn{1}{l}{}           & \multicolumn{1}{l}{}               & \multicolumn{1}{l}{}              & \multicolumn{1}{l}{}    \\

\hline
 & \multicolumn{7}{c}{Supervised Methods}                                                                                                                                                                                                \\
            \hline
DAP\cite{lampert13pami}\textsuperscript{a}                         & $\surd$                             &                                &                                    & $\surd$                        &                                    & 54.0                              & 28.5                     \\
ENS\cite{rohrbach2011evaluating}\textsuperscript{a}                & $\surd$                             & $\surd$                        &                                    & $\surd$                        &                                    & 57.4                              & 31.7                     \\
HAT\cite{al2015transfer}\textsuperscript{a}                        & $\surd$                             & $\surd$                        &                                    & $\surd$                        &                                    & 63.1                              & 38.3                     \\
ALE-attr\cite{akata2015evaluation}\textsuperscript{b}              & $\surd$                             & $\surd$                        &                                    & $\surd$                        &                                    & 66.7                              & - \\

SSE-INT\cite{zhang2015zero}\textsuperscript{c}                     & $\surd$                             & $\surd$                        &                                    & $\surd$                        &                                    & \multicolumn{1}{l}{71.5}          & \multicolumn{1}{l}{44.2} \\
SSE-ReLU\cite{zhang2015zero}\textsuperscript{c}                    & $\surd$                             & $\surd$                        &                                    & $\surd$                        &                                    & \multicolumn{1}{l}{76.3}          & \multicolumn{1}{l}{46.2} \\
SDL\cite{zhang2016zero}\textsuperscript{c}                         & $\surd$                             & $\surd$                        &                                    & $\surd$                        &                                    & \multicolumn{1}{l}{79.1}          & \multicolumn{1}{l}{50.4} \\
JFA\cite{zhang2016learning}\textsuperscript{c}                     & $\surd$                             & $\surd$                        &                                    & $\surd$                        &                                    & \multicolumn{1}{l}{\textbf{81.0}} & \multicolumn{1}{l}{\textbf{52.0}} \\

\hline
\end{tabularx}
\end{center}
\end{table*}



